Typable Fragments of Polynomial Automatic Amortized Resource Analysis

Being a fully automated technique for resource analysis, automatic amortized resource analysis (AARA) can fail in returning worst-case cost bounds of programs, fundamentally due to the undecidability of resource analysis. For programmers who are unfamiliar with the technical details of AARA, it is difficult to predict whether a program can be successfully analyzed in AARA. Motivated by this problem, this article identifies classes of programs that can be analyzed in type-based polynomial AARA. Firstly, it is shown that the set of functions that are typable in univariate polynomial AARA coincides with the complexity class PTIME. Secondly, the article presents a sufficient condition for typability that axiomatically requires every sub-expression of a given program to be polynomial-time. It is proved that this condition implies typability in multivariate polynomial AARA under some syntactic restrictions.

==> first-order_language.tex <==
% !TeX root = main.tex

\section{Overview}

\subsection{Pitfalls}
\label{sec:pitfalls in designing the notion of inherent polynomial time for univariate AARA}

Intuitively, the definition of inherent polynomial time should be less cluttered than that of inherent linear time.
This is fundamentally due to the fact that the set of polynomial functions is closed under multiplication, while the set of linear functions is now. 
As a result, if we restrict our attention to linear potential, we need to treat stepping functions' time complexity differently from the time complexity of the entire iteration.
By contrast, when working with polynomial potential, we no longer need to distinguish between the time complexity of stepping functions and that of primitive recursion.
Informally, we simply need to derive a cost bound of the stepping function, work out the length of the list on which primitive recursion has been performed, and multiply these two expressions.
Thanks to the set of polynomials being closed under multiplication, the product of these two expressions is guaranteed to be a polynomial as long as each expression is a polynomial. 

However, when working with univarite polynomial AARA, we still need to pay particular attention to stepping functions of primitive recursion. 
Specifically, the following must be avoided:
\begin{itemize}
	\item Inadvertent introduction of exponential potential;
	\item Inadvertent introduction of multivariate polynomial potential (in place of univariate polynomial potential). 
\end{itemize}
These two pitfalls are related to one another as will be explained shortly. 

To illustrate the first pitfall, consider 
\begin{equation} \label{eq:example of exponential blowup}
e := \m{rec} \; x \; \{[\,] \hookrightarrow [\,] \mid (y::\mi{ys}) \; \m{with} \; z \hookrightarrow \mi{append} \; \abra{z, z} \}. 
\end{equation}
Note that $e$ is a contrived example---it simply returns the empty list after traversing $x$ in vain. 
Although the actual running time of $e$ is $O (\abs{x})$ and hence is linear, $e$ is untypable in polynomial AARA, whether it be univariate or multivariate. 
A problem with \eqref{eq:example of exponential blowup} is that the stepping function doubles the input size.
This leads AARA to conclude that the worst-case total running time is $O (2^{\abs{x}})$, which cannot be expressed in polynomial AARA. 

On the surface, the above example suggests that we should not let the stepping function's running time have a coefficient larger than 1 with respect to $\abs{z}$. 
In other words, if $T (\abs{y}, \abs{\mi{ys}}, \abs{z})$ is the running time of $e_1$, instead of $T (\abs{y}, \abs{\mi{ys}}, \abs{z}) \leq a \abs{x} + b$ for $a > 1$, we should have a stricter bound
\begin{equation*}
	T (\abs{y}, \abs{\mi{ys}}, \abs{z}) \leq \abs{z} + b, 
\end{equation*}
where $b$ is a constant independent of $\abs{z}$ (but possibly dependent on $y$ and $\mi{ys}$). 
However, this restriction alone is not adequate, since it leaves room for the second pitfall, namely multivariate polynomial potential. 

One might conjecture that every program that is typable in multivariate polynomial AARA is also typable in univariate polynomial AARA. 
This is a plausible conjecture as, for any multivariate polynomial function $p$, there exists a univariate polynomial function $p'$ such that for all $n \in \mathbb{N}$, $p (n) \leq p' (n)$. 
For instance, a multivariate polynomial $x y$ is bounded by univariate polynomial $x^2 + y^2$. 
Thus, univariate polynomial potential is expressive enough to bound any multivariate polynomial potential. 

Nonetheless, this conjecture unfortunately does not hold. 
For example, consider 
\begin{equation} \label{eq:example of a term typable in multivariate polynomial AARA but not univariate one}
e := \m{rec} \; u \; \{[\,] \hookrightarrow \abra{w, [\,]} \mid (y::\mi{ys}) \; \m{with} \; z \hookrightarrow e_1 \}, 
\end{equation}
where
\begin{equation*}
	e_1 \equiv \m{case} \; z \; \{\abra{z_1, z_2} \hookrightarrow \m{share} \; z_1 \; \m{as} \; z_{1,1}, z_{1,2} \; \m{in} \; \abra{z_{1, 1}, \mi{append} \; \abra{z_{1, 2}, z_2}}\}. 
\end{equation*}
The arrow-type and base-type typing contexts are
\begin{equation*}
	\Sigma = \emptyset \qquad \Gamma = \{u: L (\mathbf{1}), w: L (\mathbf{1}) \}. 
\end{equation*}
Each step of primitive recursion in \eqref{eq:example of a term typable in multivariate polynomial AARA but not univariate one} produces a pair $\abra{z_1, z_2}$, and $z_1$ is prepended to $z_2$ by the stepping function $e_1$. 
For simplicity, we assume that running time accrues only by $\mi{append}$---we disregard other sources of cost. 
It is easy to see that the total running time of \eqref{eq:example of a term typable in multivariate polynomial AARA but not univariate one} is $\abs{u} \abs{w}$. 
Although it is tedious to formally prove the typability of \eqref{eq:example of a term typable in multivariate polynomial AARA but not univariate one} in multivariate polynomial AARA, we can assure the reader that it is indeed typable. 

Now let us consider whether \eqref{eq:example of a term typable in multivariate polynomial AARA but not univariate one} is typable even if we are limited to univariate polynomial potential as opposed to multivariate one. 
In $e_1$'s definition, the potential of $z_1$ is split between $z_{1,1}$ and $z_{1,2}$.
Because $z_{1,2}$ is used as the first input to $\mi{append}$, $z_{1,2}$ needs to contain positive potential.
This means that $z_{1,1}$, which acts as $z_{1}$ in the next recursive call, contains strictly less potential than $z_{1}$.
This suggests we use resource-polymorphic recursion.
However, resource-polymorphic recursion fails.
To derive a desirable cost-free resource annotation, we are required to transfer potential from $u$ to $w$, but this is impossible because $\abs{u}$ and $\abs{q}$ are independent of one another. 

In conclusion, like linear AARA, univariate polynomial AARA demands close attention to the stepping function's running time, particularly its dependence on variable $z$. 

